PaMi-VDPO: Mitigating Video Hallucinations by Prompt-Aware Multi-Instance Video Preference Learning

Direct Preference Optimization (DPO) helps reduce hallucinations in Video Multimodal Large Language Models (VLLMs), but its reliance on offline preference data limits adaptability and fails to capture true video-response misalignment. We propose Video Direct Preference Optimization (VDPO), an online preference learning framework that eliminates the need for preference annotation by leveraging video augmentations to generate rejected samples while keeping responses fixed. However, selecting effective augmentations is non-trivial, as some clips may be semantically identical to the original under specific prompts, leading to false rejections and disrupting alignment. To address this, we introduce Prompt-aware Multi-instance Learning VDPO (PaMi-VDPO), which selects augmentations based on prompt context. Instead of a single rejection, we construct a candidate set of augmented clips and apply a close-to-far selection strategy, initially ensuring all clips are semantically relevant while then prioritizing the most prompt-aware distinct clip. This allows the model to better capture meaningful visual differences, mitigating hallucinations, while avoiding false rejections, and improving alignment. PaMi-VDPOseamlessly integrates into existing VLLMs without additional parameters, GPT-4/human supervision. With only 10k SFT data, it improves the base model by 5.3% on VideoHallucer, surpassing GPT-4o, while maintaining stable performance on general video benchmarks.

==> ICCV2025-Author-Kit-Feb/sec/4_empricial.tex <==

\section{Video Preference Learning}\label{sec:empirical}

\subsection{Overall Framework}
Relying on the offline constructed preference data, the standard DPO suffer from several drawbacks,~\ie, costly annotation, outdated preference data as model training, prioritizing linguistic style alignment over true video-response misalignment.

To address these drawbacks, we introduce the video DPO (VDPO) to enforce the model to conduct the preference learning based on the videos, without the need for pre-constructed preference data.
%
As shown in Fig.~\ref{fig:motivation}~(a), VDPO consists of three steps: (i) sampling training examples,~\ie, $\{\mathbf{x}, \mathbf{y}, \mathbf{v}^w\}$, from existing SFT datasets; (ii) conducting video augmentations to the original video clip $\mathbf{v}^w$ to generate the rejected video clip $\mathbf{v}^l$;
(iii) optimizing the model,~\ie, LLaVA-OV-7B~\cite{li2024llava}, by the VDPO objective as follows:
%
\begin{equation}
 \mathcal{L}_{\text{vdpo}}=- \log \sigma \left[ \beta* \left( \mathcal{R}\left(  \mathbf{y} \mid \mathbf{x}, \mathbf{v}^w \right) - \mathcal{R}\left(  \mathbf{y} \mid \mathbf{x}, \mathbf{v}^l \right) \right)\right].
 \label{e:vdpo}
\end{equation}


\subsection{Augmentation: A Bottleneck in VDPO}


As shown in Eq.~\ref{e:vdpo}, the video input is the only variable, the construction of the rejected clip plays a key role in the performance of VDPO.
Hence, the key question is that \emph{What kinds of video augmentations are the optimal choice for video VDPO?}
%
To answer this question, we conduct an empirical study in this section to analyze the effect of different video augmentations.


\subsubsection{Experiment Setting}\label{sec:setting}

\paragraph{Sampling SFT data.} We sample a total of 10K SFT data examples from Temporal-bench\footnote{\url{https://huggingface.co/datasets/microsoft/TemporalBench}}~\cite{cai2024temporalbench} and LLaVA-Video-178k\footnote{\url{https://huggingface.co/datasets/lmms-lab/LLaVA-Video-178K}}~\cite{zhang2024videoinstructiontuningsynthetic}. The datasets are specifically chosen for allowing us to assess the performance on both temporal and visual domains.



\paragraph{Augmentations for the rejected video construction:} We select the following classical video augmentations to obtain the rejected video clip: \textbf{(1) Crop} -- randomly cropping less than 20\% of the frame from the original video; \textbf{(2) D-video} -- randomly selecting clips from another video from the training data; \textbf{(3) D-Clip} -- selecting another clip from the same long video with the original video clip. \textbf{(4) Shuffle} -- shuffling the temporal order of the original video clip; \textbf{(5) Reverse} -- reversing the original temporal order; \textbf{(6) Rate} -- sampling frames from the original video clip at a different frame rate;  \textbf{(7) Combination} -- applying two ways sampled from previous augmentation strategies.
%

To facilitate a more detailed analysis of the impact of different augmentations, we define the aforementioned augmentations into two categories as followings:

\noindent\emph{\textbf{High-similarity Augmentations:} augmentations that do not significantly alter the semantic content of the original video clip, resulting in a high similarity between the augmented and original clips.} 

\noindent\emph{\textbf{Low-similarity Augmentations:} augmentations that significantly alter the original semantic content, making it difficult or impossible to recognize the original scene or objects.} 
%

\noindent Based on the above definitions, Crop, D-Clip, Shuffle, Reverse and Rate belong to the high-similarity augmentations, while D-video and Combination belong to the low-similarity augmentations.


\paragraph{Evaluation benchmarks:} We evaluate the performance of different models on both general and hallucination benchmarks.
%
For the general benchmarks, we report the average performance of Tempcompass~\cite{liu2024tempcompass} and Video-MME~\cite{liu2024tempcompass}.
%
For the hallucination benchmarks, we report the average performance of five sub-tasks in VideoHallucer~\cite{wang2024videohallucer}.


\input{ICCV2025-Author-Kit-Feb/items/fig_analysis}

\subsubsection{Experimental Findings and Analysis}\label{sec:findings}

We report the performance gap between the baseline model LLaVA-OV-7B~\cite{li2024llava} and the baseline models trained with VDPO using different augmentations, as shown in Fig.~\ref{fig:motivation}~(b). 
%
Specifically, we initialize with the baseline model and apply each of the seven augmentations from Section~\ref{sec:setting} to generate rejected video clips for VPO training, resulting in seven distinct models. During seven times training, the augmentation is the only variable while the other settings (~\eg, dataset, epochs, learning rate) remain fixed.
%
Then, the performance difference of each model compared to the baseline is calculated. A positive difference (highlighted in \textcolor{mygreen}{green}) indicates improved performance, while a negative one (highlighted in \textcolor{red}{red}) indicates a decline.


\paragraph{Low-similarity augmentations have minimal impact on both benchmarks.} Due to the rejected video clip generated by the low-similarity augmentations having a clear semantics gap between the original video clip, the model can easily distinguish between the chosen and rejected visual inputs. Hence these chosen and rejected pairs are low-quality, and can not help the model to learn to mitigate the hallucinations.
%
To further validate this claim, we show the VPO loss over the training iterations in Fig.~\ref{fig:analysis}~(a). 
%
For clarity, we compute the mean and variance for augmentations within each group,~\ie, low-similarity and high-similarity groups.
%
It is clear that the VDPO loss training with low-similarity augmentations shows a quick convergence (\textcolor{orange}{orange curve}).



\paragraph{High-similarity augmentations boost performance on the hallucination benchmarks.} 
%
The chosen and rejected video clip pairs constructed by the high-similarity augmentations show close semantics. VDPO training with these high-quality and informative pairs would force the model to focus on subtle semantic differences, enhancing its ability to address hallucinations,~\eg, $3.5\%$ using D-Clip.

\paragraph{Instability of \ha.} We observe the instability of \has~comes from three aspects:
\begin{itemize}
    \item The performance improvements on hallucination benchmarks are very sensitive to augmentations,~\eg, D-Clip obtaining $3.5\%$ gains while Reverse only achieve $1.0\%$ improvements.
    \item The \has~often cause a clear drop on the general benchmark,~\eg, $-1.1\%$ using D-Clip.
    \item As shown in the \textcolor[HTML]{4292c9}{blue} curve in Fig.~\ref{fig:analysis}~(a), the VDPO loss of \has~coverages slowly and show large variance compared with low-similarity augmentations.
\end{itemize}

\input{ICCV2025-Author-Kit-Feb/items/fig_clean_mixed}

\paragraph{False-rejected video clips may lead to the instability of VDPO.} The effect of the same augmentation on VDPO varies across different questions.
%
As shown in Fig.~\ref{fig:analysis}~(b), we applied Reverse to the original video clip to generate a rejected one. For Question-A, the reversed video clip is the true-rejected, as the order of steps has been altered.
However, for Question-B, changing the frame order does not affect the position of the metal container, meaning that the reversed video clip is false-rejected.
%
We believe that those false-rejected video clips would destroy the alignment of pre-trained MLLMs, thus leading to the instability of \has and degrading the performance of general benchmarks.


To validate our hypothesis,  we design a controlled experiment by curating temporal-related questions from the original SFT dataset. Specifically, we leverage the GPT-4o API~\cite{gpt4o} to identify questions involving temporal reasoning (e.g., direction prediction, velocity estimation, or sequential understanding), resulting in 3K samples termed Clean data. For fair comparison, we randomly select 3K samples from the original dataset as Mixed data.
Subsequently, we apply Shuffle augmentation to train two VDPO models: one on the Clean data (resulting in the Shuffle-Clean model) and the other on the Mixed data (resulting in the Shuffle-Mixed model).
In Fig.~\ref{fig:clean_mixed}, we report the performance gap of these models compared to a baseline model on hallucination and general benchmarks, as well as examining the training loss.
%
Our results demonstrate that Shuffle-Clean significantly mitigates the instability of VDPO. This improvement stems from the fact that, for temporal-related questions in the Clean data, shuffled video clips are likely true-rejected, as shuffling disrupts the temporal information essential for accurate responses.
%
Hence, tailoring augmentation strategies to the questions to avoid false-rejected is critical for addressing instability in VDPO training.


